Bayesian Analysis of Conventional and Ultrafast Spectroscopy Data for Investigating Detachment in the MAST-Upgrade Super-X

This paper presents the application, testing and first results of a new adaptive Bayesian inference analysis which utilises conventional and ultrafast spectroscopic measurements made in the divertor chamber to investigate the divertor physics during detachment. Validation of this software is performed prior and during analyses of results, demonstrated by compelling reproductions of ideal test cases and synthetic spectroscopic measurements. Application on real diagnostic data shows strong agreement with results from previous analysis methods. We identify unprecedented success in significant advances in time and computational efficiencies. We demonstrate a $\lesssim$1000$\times$ reduction in analysis time for spectroscopic measurements from simulated and real Super-X configurations, with the analysis technique presented in this report completing in <3 minutes. Analysis of synthetic and real diagnostic measurements identifies detachment physics in agreement with previous literature.

==> content/0C-toc.tex <==
%---------------------------------------------------------------------------------
% Table of content
%---------------------------------------------------------------------------------

\newpage % Generates page break

% Table of content
\thispagestyle{empty} % Suppresses page numbers
\tableofcontents % Adds table of content
\newpage % Generates page break

% List of figures
%\thispagestyle{empty} % Suppresses page numbers
%\listoffigures % Adds list of figures; uncomment if required
%\newpage % Generates page break; uncomment if required

% List of tables
%\thispagestyle{empty} % Suppresses page numbers
%\listoftables % Adds list of tables; uncomment if required
%\newpage % Generates page break; uncomment if required


==> content/8-bibliography.tex <==
%----------------------------------------------------------------------------------------
% Bibliography
%----------------------------------------------------------------------------------------
\newpage % Includes a new page

\pagenumbering{roman} % Changes page numbering to roman page numbers
%\bibliography{literature}

\bibliography{literature.bib} % Add the filename of your bibliography
\bibliographystyle{apsr} % Defines your bibliography style
%\bibliographystyle{plain} % Defines your bibliography style

% For citing, please see this sheet: http://merkel.texture.rocks/Latex/natbib.php
